DeepBase: Deep Inspection of Neural Networks

Although deep learning models perform remarkably well across a range of tasks such as language translation and object recognition, it remains unclear what high-level logic, if any, they follow. Understanding this logic may lead to more transparency, better model design, and faster experimentation. Recent machine learning research has leveraged statistical methods to identify hidden units that behave (e.g., activate) similarly to human understandable logic, but those analyses require considerable manual effort. Our insight is that many of those studies follow a common analysis pattern, which we term Deep Neural Inspection. There is opportunity to provide a declarative abstraction to easily express, execute, and optimize them. This paper describes DeepBase, a system to inspect neural network behaviors through a unified interface. We model logic with user-provided hypothesis functions that annotate the data with high-level labels (e.g., part-of-speech tags, image captions). DeepBase lets users quickly identify individual or groups of units that have strong statistical dependencies with desired hypotheses. We discuss how DeepBase can express existing analyses, propose a set of simple and effective optimizations to speed up a standard Python implementation by up to 72x, and reproduce recent studies from the NLP literature.

==> contents/exp_acc.tex <==
\begin{figure*}[bt]
  \centering
   \begin{subfigure}[t]{.40\textwidth}
			\includegraphics[width = \columnwidth]{./experiments/exp_acc_spec_tsne_w05_group6}
			\vspace*{-.1in}
			\caption{T-SNE clustering of change in activation during verification. Each point is one unit's activation. \\ (Weight=0.5, Num Specialized=4)}
			\label{f:exp-acc-spec-tsne}
  \end{subfigure}
  \begin{subfigure}[t]{.29\textwidth}
		\centering
		\includegraphics[width = \columnwidth]{./experiments/exp_acc_spec_silhouette_group4}
		\vspace*{-.1in}
    \caption{Silhouette scores varying the number of specialized units. (Weight=0.5)}
		\label{f:exp-acc-spec-sil-group4}
  \end{subfigure}
  \begin{subfigure}[t]{.29\textwidth}
		\centering
		\includegraphics[width = \columnwidth]{./experiments/exp_acc_spec_silhouette_weight05}
		\vspace*{-.1in}
    \caption{Silhouette scores varying weight.  (Num Specialized=4)}
		\label{f:exp-acc-spec-sil-weight05}
  \end{subfigure}
	\vspace*{.1in}
	\caption{\small Verification results for parentheses detection hypothesis function.   }
	\label{f:exp-acc-spec}
\end{figure*}

\subsection{Accuracy Benchmark}
\sys is designed to quickly compute affinity scores in order to identify hidden units that are likely to learn and mimic user-understandable hypotheses.   The goal in this subsection is to understand the conditions when high affinity scores are indicative that a group of units have learned a given hypothesis.

To establish ground truth, we specially train a 16-unit RNN model by ``specializing'' a subset of units  $S\subseteq M$ to learn a specific hypothesis $h$. To do so, we introduce an auxiliary loss function $g_h$ that forces the output of the neurons in $S$ to to be close to the output of $h$.  If $g_h$ is the auxiliary loss function and $g_T$ is the loss function for $M$ based on the next character prediction task, the model's loss function is a weighed average of $g_M = w\times g_h + (1-w)\times g_T$.  This setup allows us to vary the number of specialized units $|S|$, and the specialization weight $w$ for how much the specialized units focus on learning the hypothesis.  Their defaults are $|S|=4$, $w=0.5$.

The challenge in this benchmark is that not all units in $S$ may be needed to learn a given hypothesis.  For instance, if the hypothesis is to detect the current input, then one unit may be sufficient.  In contrast, all units may be needed to learn a higher level hypothesis.    We run \sys using logistic regression with L1 regularization, return units with unit\_score above $15$, and use the perturbation-based verification method in Section~\ref{ss:verification} to assess the quality of the high scoring units.

Figure~\ref{f:exp-acc-spec-tsne} shows an example clustering of the change in activations between the baseline and treatment perturbations (colors).  The hypothesis function used to inspect the model recognizes parentheses symbols, thus the baseline perturbations swap `$($' for `$)$' or vice versa.   The treatment swaps `$($' for a number.  Units selected by \sys show clear clusters that distinguish baseline and treatment perturbations, while the change in activation for a set random units (the same number of units) overlap considerably (blue and red are indistinguishable). Figure~\ref{f:exp-acc-spec-sil-group4} summarizes the cluster separation using the Silhouette score~\cite{rousseeuw1987silhouettes} and shows higher separation than random units across all weights.  Similar results are shown when varying the number of specialized units in Figure~\ref{f:exp-acc-spec-sil-weight05}.

We also ran the above for two other hypothesis functions: predicting the current nesting level, and predicting that the current nesting level is 4.  The former hypothesis is nearly identical to the model task, and we indeed find that none of the units selected by \sys distinguish themselves from random during verification.  The latter hypothesis is ambiguous: the specialized units may simply recognize the input character $4$, or learn the nesting level.   After running verification by swapping $4$ with other numbers (baseline) or open parentheses (treatment), we find that the change in activations were indistinguishable.  Thus suggests that the specialized units learned to recognize the input $4$ rather than the logical nesting level.


\input{contents/takeaway_acc}


\if{0}
	\subsection{Boolean Expressions}

	Something about booleans

	\begin{figure}[h]
		\centering
		\includegraphics[width = .7\columnwidth]{./experiments/exp_boolean.png}
		\caption{}
		\label{f:exp-boolean}
	\end{figure}
\fi




==> contents/notations.tex <==
\begin{figure}[t]
\centering
{\small
\begin{tabular}{ll}
    \toprule
    \textbf{Notation} & \textbf{Description}\\
    \midrule
    $d\in D$     & A record in dataset $D$ is a sequence\\
                 & of symbols $[s_1,\dots,s_{n_s}]$\\
    $M\in \mathcal{M}$ & Model in input set of models $\mathcal{M}$\\
    $u\in M$     & Hidden unit in model $M$\\
    $U$          & Set of hidden units  $U \subseteq M^i$\\
    $h\in\mathcal{H}$& Hypothesis function in hypothesis library\\
    $B\in \mathbb{R}^{|n_s|}$ & Unit or hypothesis behavior\\
    $L(U,h,D)\in \mathbb{R}^{|U|}$ & Statistical measure of hidden units $U$\\
                                   & and hypothesis $h$, over dataset $D$ \\
    \bottomrule
\end{tabular}
}
\caption{Summary of notations used in the paper. }
\label{tbl:notation}
\end{figure}


==> contents/verification.tex <==
\subsection{Verification}\label{ss:verification}
This paper proposes a declarative system to express existing deep neural inspection analyses.  DNI is a data mining procedure that computes a large number of pairwise statistical measures between many groups of units and hypotheses.  When using the scores to identify high-scoring units, the decision is susceptible to multiple hypothesis testing issues and can generate false positives.  Although a complete treatment to address this problem is beyond the scope of this paper, \sys implements a perturbation-based verification procedure to ensure that the set of high scoring units indeed have higher affinity to the hypothesis function.  To do so, the procedure is akin to randomized control trials, where, for a given input record, we perturb it in a way to swap a single symbol's hypothesis behavior, and measure the difference in activations.

Formally, let $h()$ be a hypothesis function that has high affinity to a set of units $U$.  It generates a sequence of behaviors when evaluated over a sequence of symbols:
%
{\small$$h([s_1,\dots,s_{k-1},s_k]) = [b_1,\dots,b_{k-1},b_k]$$}
%
\noindent After fixing the prefix $s_1,\dots,s_{k-1}$, we want to change the $k^{th}$ symbol in two ways.  We swap it with a {\it baseline} symbol $s^b_k$ so that $b^b_k$ remains the same, and with a {\it treatment} symbol $s^t_k$ so that $b^t_k$ changes.
{\small\begin{align*}
h([s_1,\dots,s^b_k]) &= [b_1,\dots,b^b_k]\  s.t. \ b^b_k = b_k, s^b_k \ne s_k\\
h([s_1,\dots,s^t_k]) &= [b_1,\dots,b^t_k]\  s.t. \ b^t_k \ne b_k, s^t_k \ne s_k
\end{align*}}
%
Let $act(s)$ be $U$'s activation for symbol $s$, $\Delta^b_k = act(s^b_k)-act(s_k)$ be the change  activation for a baseline perturbation, and $\Delta^t_k$ be the change for a treatment perturbation.  Then the null hypothesis is that $\Delta^t_k$ and $\Delta^b_k$, across different prefixes and perturbations, are drawn from the same distribution.

For example, consider the input sentence ``He watched Rick and Morty.'', where the hypothesis function detects coordinating conjunctions (words such as ``and'', ''or'', ``but'').  We then perturb the input words in two ways. The first is consistent with the hypothesis behavior for the symbol ``\texttt{and}'', by replacing ``\texttt{and}'' with another conjunction such as ``\texttt{or}''.   The second is inconsistent with the hypothesis behavior, such as replacing ``\texttt{and}'' with ``\texttt{chicken}''.  We expect that the change in activation of the high scoring units for the replaced symbol (e.g., ``\texttt{and}'') is higher when making inconsistent than when making consistent changes.
%There may be many high scoring units and the dimensionality of the activations may be large.   Rather than a t-test, which is difficult to generalize to higher dimensions,
To quantify this, we label the activations by the consistency of the perturbation and then measure the Silhouette Score~\cite{rousseeuw1987silhouettes}, which scores the difference between the within- and between-cluster distances.

Our verification technique is based on analyzing the effects of input perturbations on unit activations, however there are a number of other possible verification techniques.  For instance, by perturbing the model using ablation~\cite{morcos2018importance,karpathy2015visualizing} (removing the high scoring units and retraining the model) and measuring its effects on the model's output.  We leave an exploration of these extensions to future work.




